Search for {\Theta^+} in KLp \to K+n reaction in KLF at JLab

The possibility of the existence of multiquark hadrons made of 4-quark for mesons and 5-quark for baryons was predicted by Gell-Mann in Ref. [1]. The renewed interest for the search of exotic pentaquark states was initiated by the paper by Diakonov, Petrov, and Polyakov in Ref. [2]. The 2003 experimental reports on the observation of {\Theta^+} pentaquark with a uudd{\bar s} quark content created a big excitement and many following experiments have reported its observation [3]. After high-statistics experiments at JLab, which did not confirm previous claims by the CLAS collaboration, the community concluded that the {\Theta^+} pentaquark either does not exist at all or has an extremely small cross section, making it currently unobserved. There were different review papers on this subject, either questioning the existence of the {\Theta^+} or attempting to explain the reasons why reaching a conclusion based on production experiments is challenging [4]. To address the challenge of minimal 3-body final states, a formation experiment with a projectile kaon beam is proposed. Below, we discuss how the {\Theta^+} could be observed in the KLp \to {\Theta^+} \to {K^+}n reaction in the KLF experiment at JLab [5].

==> author_list.tex <==
\author{\mbox{Moskov~J.~Amaryan}}
\altaffiliation{\texttt{mamaryan@odu.edu}}
\affiliation{Department of Physics, Old Dominion University, Norfolk, Virginia 23529, USA}

\author{\mbox{Shu~Hirama}}
\altaffiliation{\texttt{hirama.s.aa@m.titech.ac.jp}}
\affiliation{Department of Physics, Tokyo Institute of Technology, Megro, Tokyo 152-8551, Japan}

\author{\mbox{Daisuke~Jido}}
\altaffiliation{\texttt{jido@th.phys.titech.ac.jp}}
\affiliation{Department of Physics, Tokyo Institute of Technology, Megro, Tokyo 152-8551, Japan}

\author{\mbox{Igor~I.~Strakovsky}}
\altaffiliation{\texttt{igor@gwu.edu}}
\affiliation{Institute for Nuclear Studies, Department of Physics, 
    The George Washington University, Washington, DC 20052, USA}

\noaffiliation


==> references.tex <==
\begin{thebibliography}{99}
\bibitem{Gell-Mann:1964ewy}
   M.~Gell-Mann,
   ``A schematic model of baryons and mesons,''
   Phys.\ Lett.\ \textbf{8}, 214 (1964).
\bibitem{Diakonov:1997mm}
   D.~Diakonov, V.~Petrov, and M.~V.~Polyakov,
   ``Exotic anti-decuplet of baryons: Prediction from chiral solitons,''
   Z.\ Phys.\ A\ \textbf{359}, 305 (1997).
\bibitem{Hicks:2012zz}
   K.~H.~Hicks,
   ``On the conundrum of the pentaquark,''
   Eur.\ Phys.\ J.\ H\ \textbf{37}, 1 (2012).
\bibitem{Amaryan:2022iij}
   M.~Amaryan,
   ``History and geography of light pentaquark searches: challenges and pitfalls,''
   Eur.\ Phys.\ J.\ Plus\ \textbf{137}, 684 (2022).
\bibitem{KLF:2020gai}
   M.~Amaryan \textit{et al.} [KLF Collaboration],
   ``Strange hadron spectroscopy with secondary KL beam in Hall~D,''
   [arXiv:2008.08215 [nucl-ex]].
\bibitem{ParticleDataGroup:2022pth}
   R.~L.~Workman \textit{et al.} [Particle Data Group],
   ``Review of Particle Physics,''
   Prog.\ Theor.\ Exp.\ Phys.\ \textbf{2022}, 083C01 (2022).
\bibitem{LHCb:2019kea}
   R.~Aaij \textit{et al.} [LHCb Collaboration],
   ``Observation of a narrow pentaquark state, $P_c(4312)^+$, and of two-peak structure of the $P_c(4450)^+$,''
   Phys.\ Rev.\ Lett.\ \textbf{122}, 222001 (2019).
\bibitem{LEPS:2003wug}
   T.~Nakano \textit{et al.} [LEPS Collaboration],
   ``Evidence for a narrow S = +1 baryon resonance in photoproduction from the neutron,''
   Phys.\ Rev.\ Lett.\ \textbf{91}, 012002 (2003).
\bibitem{DIANA:2003uet}
   V.~V.~Barmin \textit{et al.} [DIANA Collaboration],
   ``Observation of a baryon resonance with positive strangeness in $K^+$ collisions with Xe nuclei,''
   Yad.\ Fiz.\ \textbf{66}, 1763 (2003) 
   [Phys.\ Atom.\ Nucl.\ \textbf{66}, 1715 (2003)].
\bibitem{LRP:2023}
   Long Range Plan (LPR2023), \\
   https://nuclearsciencefuture.org/wp-content/uploads/2023/11/NSAC-LRP-2023-v1.3.pdf 
\bibitem{koto:2006}
   T.~Yamanaka \textit{et al.} [KOTO Collaboration], 
   ``Proposal for $K_L \to \pi^0 \nu \bar{\nu}$ experiment at J-PARC,'' J-PARC Experimental Proposal, E14 (2006).
\bibitem{Koniuk:1979vw}
   R.~Koniuk and N.~Isgur,
   ``Where have all the resonances gone? An analysis of baryon couplings in a quark model with chromodynamics,''
   Phys.\ Rev.\ Lett.\ \textbf{44}, 845 (1980).
\bibitem{Thiel:2020eqn}
   A.~Thiel and E.~Klempt,
   ``Highlights of the spectroscopy of hyperons and cascade baryons,''
   [arXiv:2005.06971 [nucl-ex]].
\bibitem{Brandenburg:1972pm}
   G.~W.~Brandenburg \textit{et al.}
   ``Production of K0(L) mesons and neutrons from electron on beryllium above 10-GeV,''
   Phys.\ Rev.\ D\ \textbf{7}, 708 (1973).
\bibitem{Hyslop:1992cs}
   J.~S.~Hyslop, R.~A.~Arndt, L.~D.~Roper, and R.~L.~Workman,
   ``Partial wave analysis of K+ nucleon scattering,''
   Phys.\ Rev.\ D\ \textbf{46}, 961 (1992).
\bibitem{Arndt:2003xz}
   R.~A.~Arndt, I.~I.~Strakovsky, and R.~L.~Workman,
   ``K+ nucleon scattering and exotic S = +1 baryons,''
   Phys.\ Rev.\ C\ \textbf{68}, 042201 (2003);
   [erratum: Phys.\ Rev.\ C\ \textbf{69}, 019901 (2004)].
\bibitem{DIANA:2013mhv}
   V.~V.~Barmin \textit{et al.} [DIANA Collaboration],
   ``Observation of a narrow baryon resonance with positive strangeness formed in $K^+$Xe collisions,''
   Phys.\ Rev.\ C\ \textbf{89}, 045204 (2014).
\bibitem{Iizawa:2023xsi}
   Y.~Iizawa, D.~Jido, and S.~H\"ubsch,
   ``$K^+ N$ elastic scatterings for estimation of in-medium quark condensate with strange quarks,''
   [arXiv:2308.09397 [hep-ph]].
\bibitem{Cahn:2003wq}
   R.~N.~Cahn and G.~H.~Trilling,
   ``Experimental limits on the width of the reported Theta(1540)+,''
   Phys.\ Rev.\ D\ \textbf{69}, 011501 (2004).
\bibitem{Ahn:2023hiu}
   J.~K.~Ahn and S.~H.~Kim,
   ``Search for $\Theta ^+$ in $K^+d\rightarrow K^0pp$ reaction at J-PARC,''
   J.\ Korean\ Phys.\ Soc.\ \textbf{82}, 579 (2023).
\bibitem{Migdal:1955ab}
    A.~B.~Migdal, 
    ``The theory of nuclear reactions with production of slow particles,''
    Zh.\ Eksp.\ Teor.\ Fiz.\ \textbf{28}, 3 (1955) [Sov.\ Phys.\ JETP\ \textbf{1}, 2 (1955)].
\bibitem{Watson:1952ji}
    K.~M.~Watson,
    ``The effect of final state interactions on reaction cross-sections,''
    Phys.\ Rev.\ \textbf{88}, 1163 (1952).
%\bibitem{Azimov:2007hq}
%   Y.~I.~Azimov, K.~Goeke, and I.~Strakovsky,
%   ``An Explanation why the Theta+ is seen in some experiments and not in others,''
%   Phys.\ Rev.\ D\ \textbf{76}, 074013 (2007).
\end{thebibliography}

